Collaborative Development of NLP models

Despite substantial advancements, Natural Language Processing (NLP) models often require post-training adjustments to enforce business rules, rectify undesired behavior, and align with user values. These adjustments involve operationalizing "concepts"--dictating desired model responses to certain inputs. However, it's difficult for a single entity to enumerate and define all possible concepts, indicating a need for a multi-user, collaborative model alignment framework. Moreover, the exhaustive delineation of a concept is challenging, and an improper approach can create shortcuts or interfere with original data or other concepts. To address these challenges, we introduce CoDev, a framework that enables multi-user interaction with the model, thereby mitigating individual limitations. CoDev aids users in operationalizing their concepts using Large Language Models, and relying on the principle that NLP models exhibit simpler behaviors in local regions. Our main insight is learning a \emph{local} model for each concept, and a \emph{global} model to integrate the original data with all concepts. We then steer a large language model to generate instances within concept boundaries where local and global disagree. Our experiments show CoDev is effective at helping multiple users operationalize concepts and avoid interference for a variety of scenarios, tasks, and models.

==> challanges.tex <==
\section{Challenges}
\begin{enumerate}
    \item How experts can communicate their concept with the system? training examples? writing specification? 
    \item How can we provide certification? (e.g, RAI incident generalization).
    \item Experts can have conflicts with each other, how can we address that?
    \item how about conflicts between experts and $C_0$.
\end{enumerate}

==> disagreement_accuracy_relation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/disagreement_accuracy_relation.png}
    \caption{Accuracy and the ratio of disagreement in the unlabeled pool in MNLI task with downard and upward monotone as concepts.
    As the model learns different concepts (higher accuracy) the ratio of disagreement between local and global decreases. \fk{remove accuracy from the axis}}
    \label{fig:disagreement_accuracy_relation}
\end{figure}

==> experiments.tex <==
\section{Experiments}
In \ref{sec:unlabeled} we run experiments with a simplified version of CoDev, where instead of using GPT-3 as a generator we iteratively select examples from an unlabeled pool for labeling.
Since we do not need users in the loop, this allows us to compare the data selection mechanism of CoDev to baselines such as random selection and uncertainty sampling (noting that a generator is needed to actually operationalize a concept in realistic scenarios).
In \ref{sec:oracle} we add GPT-3 back as a generator and show \method{} can operationalize a concept even when we start from a biased set.
Finally, in \ref{sec:full} we evaluate CoDev with users in the loop, and compare it to AdaTest \cite{ribeiro2022adaptive}, a state-of-the-art tool for debugging NLP models that also uses GPT-3.

% First we show \method{} outperfomrs AdaTest \cite{ribeiro2022adaptive}, a state-of-the-art tool for debugging NLP models that also uses GPT-3 by finding more bugs in and fixing them without interference.
% We then show \method{} \method{} can operationalize a concept even when we start from a biased set.
% Finally, to compare the data selection mechanism of CoDev to baselines such as random selection and uncertainty sampling we run experiments with a simplified version of CoDev, where instead of using GPT-3 as a generator we iteratively select examples from an unlabeled pool for labeling.

\subsection{CoDev with unlabeled data}
\label{sec:unlabeled}
We adapt \method{} so that it selects instances from a pool of unlabeled data based on the disagreement score rather than using GPT-3 as a generator (lines 5-6 in Algorithm \ref{alg:concept}).
We compare \method{} with two data selection baselines: random selection and uncertainty sampling \cite{lewis1995sequential, nguyen2022measure}.
Each method selects a batch of $50$ examples per iteration (CoDev selects examples randomly in the first batch), after which models are retrained.

\input{single_active_random_fig}
{\bf Operationalizing a concept.}
We use RoBERTa-Large \cite{liu2019roberta} finetuned on MNLI (binary) \cite{wang2018glue} as a base model, and use the downward-monotone concept from an NLI monotonicity dataset \cite{yanaka2020neural} as a pool of unlabeled data. The base model starts with high accuracy on the base validation dataset (93.5\%), and low accuracy on the concept (23.5\%).
We present accuracy on the concept over iterations in Figure \ref{fig:single_active_random_fig}. While accuracy on the base data remains constant throghout iterations, CoDev's disagreement-based sampling is more efficient than uncertainty sampling or random selection.

\input{multi_active_random_table}
{\bf Avoiding interference.}
%setup
In order to evaluate interference between concepts, we try to learn various concepts simultaneously.
We use the same NLI model and concept as the previous paragraph, and add upward monotone \cite{yanaka2020neural} as an additional concept. We also use RoBERTa-LARGE finetuned on the ``digital ebook'' category of Amazon Reviews as a base model, and use 4 additional product categories as concepts to be learned (pet-product, home, home-improvement, and wireless).
We run 10 iterations of each method, with random sampling and uncertainty sampling selecting an equal number of instances from each concept per round. 
%result 
Table~\ref{tab:simul_multi} shows the per-concept average and worst case accuracy of each method, where we note that \method{} produces better models on average. 


\input{biased_table}
\input{interference_table}
\subsection{CoDev with biased seed data}
\label{sec:oracle}
Here we add GPT-3 back as a generator, but avoid the need of user labels by training a high accuracy model as an oracle to simulate user labels.
As an oracle, we train RoBERTa-Large on the whole Amazon Review dataset where we only keep reviews with rating $5$ (positive sentiment) and rating $1$ (negative sentiment). The accuracy of oracle on validation dataset is 98.6\%.
We train a weaker base model by finetuning BERT-base-uncased on reviews that contain the word ``install''.

Our simulated concept consists of reviews containing the phrases ``battery life'' or ``my skin'' (from now on, we refer to this concept as SB). We split these reviews into a development set (to initialize \method{} and baselines) and a test set.
We simulate the scenario where the user starts with a biased subset of the concept, by initializing the concept with $10$ instances such that instances with ``battery life'' are always positive, and those with ``my skin'' are always negative.
We then run \method{} with the oracle for $5$ rounds adding $10$ data points in each round.
As shown in \reftab{biased}, CoDev is able to achieve high accuracy on all of SB, despite starting with a biased sample, while the same number of random instances from biased SB increases accuracy on it to the detriment on accuracy on the whole concept.
Qualitatively, GPT-3 starts generating in-concept instances without the bias, as that is where the local concept model disagrees with the base model.
This controlled experiment illustrates how a generator focused on disagreements can be helpful in exploring the boundaries of concepts, even when we start from a biased sample. 


\subsection{CoDev with real users}
\label{sec:full}
{\bf Operationalizing concepts.}
We compare \method{} to AdaTest \cite{ribeiro2022adaptive}, using data and concepts made available by \citet{ribeiro2022adaptive}.
They finetune a RoBERTa-Large model on the Quora Question Pairs (QQP) dataset (validation accuracy 92.2\%), and then iteratively add data with GPT-3  (adaptively trying to find failures) until they ``fix'' $6$ concepts from CheckList tests \cite{ribeiro2020beyond}.
\citet{ribeiro2022adaptive} run adaptive testing ``until finding failures becomes qualitatively difficult''.

For each concept, we initialize \method{} with their generated data as $D_i$.
Even though the model has been `debugged' with AdaTest, \method{} quickly reveals $\approx 5$ semantically meaningful sub-categories of bugs for each concept (with many failures within each sub-category).
We show a few examples from different sub-categories in Table~\ref{tab:checklist_examples_codev}, which illustrate that AdaTest had not yet operationalized various regions of concepts where the model was still failing.

\input{qual_analysis}

{\bf Interference.}
We now compare \method{} with AdaTest in terms of handling interference.
To do so, we pick pairs of concepts $C_{orig}$, $C_{new}$ that might cause interference with one another, but that were debugged and reported as ``fixed'' by \citet{ribeiro2022adaptive}. We then run \method{} on these pairs, noting that the output of both AdaTest and \method{} are small concept datasets $D_{orig}$ and $D_{new}$.

We then train two models for each method, one finetuned on $D_{orig}$ and one finetuned on the union of $D_{orig}$ and $D_{new}$. Finally, we generate new data from $P_{orig}$ and manually label $50$ instances where there is disagreement between the models, to check if adding $D_{new}$ caused interference on $P_{orig}$. 
We present the proportion of sentences that were broken (right to wrong) or fixed (wrong to right) when the new concept is added in Table \ref{tab:adatest_codev_conflict}, disregarding instances that are invalid, out of domain, or for which the label is unclear.
The top pair seems more liable to interference between concepts, but we note that AdaTest data results in much more interference than \method{} data. In the bottom pair, adding a concept with \method{} actually improves the original concept more often than interferes with it, while AdaTest data has a neutral effect.


{\bf Pilot Study (qualitative).}
We conducted a pilot study with four users (one computer scientist and three with no prior knowledge of AI) who used \method{} to align a model within their chosen concept in either sentiment analysis or toxicity task.
Each participant interacted with \method{} for 5-7 rounds, and reported an improved alignment in their concept and an increase in sentence complexity over time.

For the Sentiment \& Islam, the user-provided seed data matched the global model perfectly, indicating no initial bugs.
However, in the first round of using \method{}, some disagreement were found between the fitted local model and the global model. The user identified some of these as bugs in the global model (e.g. ``Alice practices Islam daily" where the global model predicted negative) and some as bugs in the local model (e.g. ``Alice is a radical Islamist" where the local model predicted neutral).
As the user made repeated adjustments to both models, the disagreements gradually centered around the concept boundaries, reaching a point where users could no longer determine the correct behavior.
This pattern of initial misalignment correction followed by uncertainty in label determination was consistent across all users, suggesting successful concept operationalization in clear label regions. Table~\ref{tab:operationalize_qual} provides examples of user interactions with \method{}.





==> extra.tex <==
\subsection{Goals in each iteration between user and the model}
In each interaction between the model and the users we like to achive the following 4 goals:
\begin{enumerate}
    \item understand the distribution of the user $\sP_i$ (i.e., being able to classify the points for the user concept so the system be able to show related points in the future).
    \item understanding the labeling function of the user $f_i$ (i.e., being able to classify points from $\sP_i$)
\end{enumerate}
\noindent There are two points that need to make decision:
\begin{enumerate}
    \item what examples we should put in the generator?
    \item what examples we should show to the user?
\end{enumerate}



\subsection{Adjusting the model}
    % $M$ uses $\sG$ with active learning methods to generate data points with most uncertainty 
In this step, we use Active learning methods (uncertainty sampling? hypothesis disagreement?) to find the right classifier that is not in conflict with the concept $C_i$.

\paragraph{Proposal 0}
\begin{enumerate}
    \item Choose the most uncertain labeled data points and use $\sG$ to generate data points near them. 
    \item choose data points with the most uncertainty and put them in the set $q$
    \item use $\sG$ on $q$ to generate more uncertain data points and go to step 2. \fk{for K times?}
    \item retrain the model and go to step 1. \fk {for K times?}
\end{enumerate}


\fk{what are the benefits of this step?
\begin{enumerate}
    \item It reduces the number of iteration/retraining (we assume retraining the model is costly)
    \item it might find some errors/edge cases that the user cannot find? 
\end{enumerate}}


\subsection{Iteration}
In this step, we retrain the underlying model using $D_0$ and the new collected dataset $D_i$. We then go back to step 2 until no more error is reported by the user $u_i$. Let's call the new model $M_i$.

\begin{proposition}
Marco's conjecture: If we do step 2, then retrain the model and do step 2 again the set of data points are equal to the set of data points of step 3. 
\end{proposition}
\begin{proof}
Seems correct, if 1) we bound ourselves to only points from $\sP_i$ and 2) use uncertainty sampling for active learning.
\end{proof}


\begin{proposition}
Under condition X, the model $M_i$ is certified with respect to the concept $C_i$.
\end{proposition}

\begin{proof}
\fk{There is a lot of sample bias here! Both from the user and from the model! I'm not sure if we can come up with good generalization bound unless we put crazy amount of constraints here! There are many amazing active learning experts in Microsoft. Should we talk to them? (Alekh has left MSR for google :'()}
\end{proof}

\begin{proposition}
Under condition X, we only need to retrain the model $Y$ times before certification.
\end{proposition}

\begin{proof}
\fk{I have no idea how many times usually it takes! should look at the experiments on the paper. But I think active learning might reduce this number}
\end{proof}

\begin{proposition}
Under condition X proposal 0 will converge in Y steps.
\end{proposition}
\begin{proof}\fk{
convergence should be easy I don't think loop will happen. However, understanding number of steps should be hard and useless :D}
\end{proof}

The proposal 0 needs a lot of steps and each user should interact with the system many times. Furthermore, since the interaction are sequential this can takes a lot of time to certify everything. How can we improve this?




\paragraph{Main question:} How to keep track of boundary of all concepts so we ask a user to interact with the system only if necessary (instead of asking the user  every time that the model changes). 

\begin{proposition}
For $k$ users, the proposal X result in a certified model with respect to all concepts with $\sO(k^2)$ interactions. 
\end{proposition}

\begin{proof}
\fk {no idea :-)}
\end{proof}


\paragraph{Proposal 1.}
In this proposal we change the Step 2 such that for each user $u_i$ in Step 2, in addition to find bugs in the model ($M_0$), the system uses $\sG$ to find potential conflicts with previous concepts. 
\begin{enumerate}
    \item For each concept $j$ and any different pair of labels ($y_0$, $y_1$) find a classifier to classify points of concept $i$ with label $y_0$ from the points of concept $j$ with label $y_1$.
    \item Use $\sG$ to generate data points near the set of data points from concept $i$ and choose the data points near the boundary.
    \item ask $u_i$ to choose data points in her concept (modify if necessary) and add the new data points to the sequence and go to step 2.
\end{enumerate}


We believe that with this proposal when $u_i$ changes the model then $u_i$ do not need to change the model again. Therefore, it reduces the number of interactions.



\paragraph{Proposal 2.}
Finding a classifier between two set of data points might not be very effective. Here we assume $\sG$ has another ability. Given two set of data points $q_1$ and $q_2$ we assume $\sG$ can generate $x$ such that $x$ is close to $q_1$ and $q_2$ (previous work on in-filling?). Using this new ability we can improve the step 1 and 2 on Proposal 1.
% \begin{enumerate}
%     \item start from the first set, Use $\sG$ to generate data points near the set of data points.
%     \item choose data points that are near the boundary (ask human for consistency), add the new data points to the sequence and go to step 2.
% \end{enumerate}

==> limitation_extended.tex <==
\section{Extended Version of Broader Impact and Limitations}
CoDev aids in operationalizing concepts without filtering the values a user wishes the model to align with.
This might inadvertently allow a malicious user to encode harmful behavior into the NLP model, a risk for which we currently have no safeguards. 


CoDev's functionality greatly depends on the interconnectedness of data points within the generator (we used GPT-3 in our experiments). Consequently, in situations where we lack data for specific concepts, CoDev may not assist users in putting their concept into action, an example being the operationalization of concepts in low resource languages.

It is important to mention that we do not employ LLM for labeling tasks, hence the biases present in the Language Model (LLM) will not propagate into our model. Indeed, CoDev can be used as a tool to tackle these biases in the LLM.
However, if biases exist within the LLM (e.g., sentences pertaining to certain religious contexts being closely related to those discussing violence) the user may need to engage more intensively with the system to accurately operatinalize the concept. On the other hand, a user working with a concept without any particular bias in the LLM will require less effort.


In terms of interference management, we only handled interference that arises from machine learning shortcomings and can be addressed by adding more data. However, there might be literal disagreements between users (i.e., two users assign different labels to the \emph{same} sentence). Although our method can surface such disagreements, we lack a definitive solution to resolve disagreements between users. 

Finally, our theoretical framework is limited but our goal was to gain some initial insights into why interference occurs and estimates the number of instances required to address it.

Tackling these challenges - safeguarding against malicious users, resolving literal disagreements, and conducting a more comprehensive theoretical analysis of alignment - are valuable directions for future research.

==> old_experiment.tex <==

----------------------------------
\subsection{Operationalizing and debugging concepts}
\label{sec:debugging-experiment}
% \input{finding_bugs_table}
\paragraph{Finding bugs.} We compare the performance of \method{} against two previous works, AdaTest \cite{ribeiro2022adaptive} and CheckList \cite{ribeiro2020beyond}.
For our experiments, we fine-tuned a RoBERTa-Large model for duplicate question detection on the Quora Question Pairs (QQP) dataset. 
The base model achieved 92.2\% accuracy on the test data. However, CheckList identified 39 categories in which the model had accuracy less than 80\%. They exposed the bugs using templates, and proposed using data from these templates to fix the bugs.
In AdaTest, the authors chose 6 distinct high failure topics and iteratively worked with the model to expose more bugs in those concepts, fine-tuning the model on the collected data until finding bugs became qualitatively difficult.

Using \method{}, we were able to find 5 or more categories of bugs in each concept, demonstrating the superior bug-finding abilities of our method compared to AdaTest and CheckList. Table~\ref{tab:checklist_examples} shows two examples of concepts along with the bugs found by \method{}. It is worth noting that we do not report accuracy as after finding one bug, \method{} can generate a large number of bugs through paraphrasing with the help of LLMs. 
% As we continue to use \method{} in multiple rounds, the examples become more challenging as the model attempts to understand the user's concept of duplication.

Table~\ref{tab:checklist_examples} illustrates two examples of concepts along with the bugs identified by \method{}. It is important to note that we do not report accuracy as after identifying a single bug, \method{} can generate a large number of bugs through paraphrasing with the help of LLMs. As we continue to use \method{} in multiple rounds, the examples become increasingly challenging as the model attempts to understand the user's concept of duplication. For example, after round 5, the model may generate examples such as \texttt{How can I become a powerful person? | How can I make myself stronger?} or \texttt{How can I be more healthy? | How can I become less ill?}, at which point the user must decide the exact definition of duplication.



% \input{biased_table}
\paragraph{Operationalizing concepts with biased seed.} 
We now illustrate the ability of \method{} to operationalize a concept even when the seed data is biased. We use a sentiment analysis task on the Amazon review dataset, filtering for only reviews with a rating of 0 as negative and reviews with a rating of 5 as positive. We fine-tune Roberta-Large on this dataset, achieving 98.6\% accuracy and using it as an oracle.

To create a biased dataset, we only choose reviews that contain the phrase "battery life" for positive reviews and "my skin" for negative reviews (referred to as the Skin-Battery (SB) dataset). We then train a weak model, BERT-Uncased, on reviews containing the word "install" to serve as the base model.

The results, as shown in Table~\ref{tab:biased}, demonstrate that the collecting more data performs only increase accuracy on the biased SB dataset but decrease the accuracy on the whole SB dataset. 
However, when using \method{} with the oracle in a loop for 5 iterations, high accuracy is achieved on the whole SB dataset even when only using 10 biased data points.

This experiment highlights the effectiveness of \method{} in mitigating bias in the dataset and achieving better performance on the whole concept. 
The results demonstrate that \method{} can improve the generalization ability of the model and prevent it from being affected by bias in the training data, a common issue in data collection.

% \input{qual_analysis}
\paragraph{Qualitative analysis of Operationalization.} To qualitatively analyse the operationalization of \method{} we run a pilot study with four users (one computer scientist and three with no prior knowledge of AI).
We ask them to choose a task (either sentiment or toxicity) and choose a topic that they want to align the model with it. 
Each participant interacted with \method{} for a period of 5-7 rounds, and reported a perceived alignment of the local model with their concept as well as an increase in sentence complexity throughout the interaction.
% Some of the user in the final rounds could not make a decision about if some sentence is toxic or not. 
Table~\ref{tab:operationalize_qual} shows some examples of user's interaction with \method{}. 


% \input{single_active_random_fig}
\paragraph{Comparison with Active learning and random selection.}
We can adapt \method{} to work with pool of unlabeled data instead of real user in the loop. 
When we have access to pool of unlabeled data for a concept every selected data point is in concept and the only information that we need is the label. 
Thus, \method{} can be viewed as an effective way of choosing the most informative data points from a novel concept for labeling. 
Using this adaptation, we evaluate the performance of \method{} against two baseline methods: random selection and active learning. 

We chose the downward-monotone as a concept and work with downward-montone dataset \cite{yanaka2020neural} as the pool of unlabeled data.
For the base model we fine-tuned RoBERTa-Large on MNLI dataset (two-way) which is known to have poor accuracy on downward-monotone examples (25.3\%) \cite{yanaka2020neural}.

%how does method work
We first select $50$ random example from downward monotone as the seed data, and fine-tune base model on them for local model and fine-tune base model on seed in addition to same amount of data from training data for the global model. 
We continue for $6$ rounds and at each step we select $50$ examples with the highest disagreement between local and global function. 

%how does baselien work
For the baselines, random selection samples $50$ data points randomly from downward-monotone at each round.
Active learning samples $50$ data points with the lowest confidence values \cite{lewis1995sequential,nguyen2022measure}. The confidence value of a data point is  $1-P(y_1 \mid x)$ where $y_1$ is the highest prediction for $x$.

%result and conclusion
Figure~\ref{fig:single_active_random_fig} shows that \method{} outperforms active learning and random selection in this task. 
This experiment demonstrates that the data selection component of \method{} can effectively identify and select data points that are important for learning a new concept in the context of the current global model, since \method{} consider the overlap between original model and new concept, it can learn the new concept faster than the baselines. 



\subsection{Handling interference}
\label{sec:interference-experiment}
\paragraph{Comparison with AdaTest.}
%goal
We now show \method{}  handles interference between different concepts better than AdaTest.
%setup pair selection
We first select two pairs of concepts from concepts in the CheckList for question duplicate detection.
We chose ``X person = not antonym(X) person'' as concept 1 and ``Modifiers changes question intent'' as concept 2. 
We chose these two concepts due to their potential to interfere with one another, with the concept 1 having a bias towards predicting duplicate and concept 2 having a bias towards predicting duplicate. 


%setup fine-tunning
For each method (AdaTest and \method{}) , we fine-tuned two models: one using data from interactions for concept 1 (old model) and another using data from interaction for both concepts (new model).
Our aim is to compare how well the new model performs on the old concept. In other word, we want to check if the new concept introduces new bugs or fixes some bugs in the old concept. 

%how we did comparison
To conduct the comparison between the old and new models, we use \method{} technique to generate sentences that two model disagree upon as explained in Section~\ref{sec:disagreement}. 
For each method, we generate and then manually label $50$ data points that the old and new model disagree categorizing them as wrong format, out of domain, introducing new bugs, fixing existing bugs, or unclear. 

%run experiment for another pair (I did nto say this at first since things get confusing)
We run the same analysis for another pair that are more similar to each other. 
We chose  `` X  = synoym (X) '' as concept 1 and `` more X = less antonym (X)'' as concept 2, these two concepts seems to be more aligned with each other and as we see will not have interfere with each other a lot.

%result
Table~\ref{tab:adatest_codev_conflict} shows the percentage of fixed or broken examples when comparing old and new models in the domain of old model.
\method{} outperforms AdaTest in handling the interference caused by a new concept in the domain of an old concept when concepts interfere with each other (top rows). We did not observe a lot of interference when the concepts are similar to each other (bottom rows). 


% We choose these two concepts due to their potential to interfere with one another, with the first having a bias towards predicting not-duplicate and the second having a bias towards predicting duplicate.
% We selected two topics from the concepts in the CheckList for question duplicate detection: 
%  ``Modifiers changes question intent'' and 
% (2) ``X person = not antonym(X) person'' (see \reftab{checklist_examples} for examples). 

% We did the same procedure with 
% old concept: `` X person = not antonym (X) '' and 
% new concept= `` more X = less antonym (X)''. 
% Rate of interference is lower for these two pairs and they actually improve each other's performance as they are more aligned with each other. 


% \input{multi_active_random_table}
\paragraph{Comparison with Active learning and random selection.}
%setup
Similar to the last section, we now compare \method{} to active learning and random selection when we have access to an unlabeled pool of data.
In MNLI task, we chose downward and upward monotone as concepts and trained Roberta-Large on the original data for the base-model. 
In Amazon Review we chose 4 product category (pet-product, home, home-improvement, and wireless) as the concepts and train Roberta-Large on another product category (digital ebooks) for the base models. We only work with reviews with ranting 1 and 2  negative and 3 and 4 as positive. 
% \footnote{We trained Roberta-large on each product category and observe its performance on other categories, we then choose digital-ebook since it has low performance on these products comparing to have a personalized model for each one of these products}
%

\fk{I gave up here}
%setup of method
\method{} as described in Section~\ref{final-algo} starts with $50$ samples randomly from each concept and train a local model it then continue for 10 rounds and in each round we use $\min(50, \#disagreement)$ to label and then fine-tune the model and continue to the next round. 

%baselines
Random data collection, simply chose 1000 samples from each concept and 1000 samples from the orignal concept and fine-tune the base model on them.
Active learning choose the top 50 data point with highest uncertainty from each concept (including original) update the model and continue to the next round.


%result 
Table~\ref{tab:my_label} shows the overall average and the worst-case accuracy among concepts. We trained each model 10 times and report the average. 
\method{} outperforms random collection 
Figure~\ref{fig:disagreement_accuracy_relation} shows how \method{} deals with interference between model and change the amount of labeling among different concepts. 

% \input{disagreement_accuracy_relation}
% \input{interference_table}

==> old_method.tex <==
\section{Method}
In order to reach our goal (\ref{eqn:goal}), we are going to create $k$ dataset $D_{1:k}$ such that model trained on all these dataset have good performance on every domain. 
In Section~\ref{sec:debugging}, we show how \method{} collaborate with a single user to conceptualize their concept within the context of the model which includes identifying, generalizing, and fixing \emph{bugs} in the model; and in Section~\ref{sec:interference}, we demonstrate how \method{} effectively manage interference between concepts and allowing user to collaboratively update the model. 

\subsection{Sampling from the concept}

The main challenge is that we cannot sample from $\sP_i$.
In order to address this challenge we use the generator $\sG$ to create a Markov chain to simulate a random walk within the user's distribution ($\sP_i$). 
Specifically, we begin with a user-provided seed data point $x$ and use it as a prompt for $\sG$ to generate a new data point $x'$. If $\sP_i(x') >0$, we accept $x'$, otherwise we remain at $x$ and repeat the process. 

%connectivity is important
In Appendix~\ref{sec:app} we study conditions under which the stationary distribution of this Markov chain is $P_i$. However, note that we do not need this condition to find bugs during random walk we only need connectivity according to the transition function $\sP'$ which means for any $x_1, x_n \in C_i$ there exists $x_2, \dots, x_{n-1} \in C_i$ such that $\Pi_{i=1}^{n-1} \sP'(x_{i+1} \mid x_{i}) > 0$, Given this condition we will find bugs after enough explorations. 

%exploration -> more rejection but cover more of user domain, explotation -> less reject, less query
\paragraph{Uncovered error.} 
% In order to make the $\sG$ transitions more aligned with the $\sP_i$ we can do a better prompt engineering by adding some information about the concept to the prompt, or adding multiple data points instead of only one. 
Depending on the prompt we can make the probability of generating in-domain for a concept lower but having high recall (e.g., only using 1-2 data points as prompt). Or, we can make the prompt more specific (e.g., adding some info and 10 data points) and increase the probability of generation in-domain but decrease the recall.  


% We start by inferring a model that has low error on the dataset collected from $\sP_0$ using a loss function (we can also assume $M_0$ is given to us).
% \todo[inline]{Maye you could have $M_0$ just be part of the setup, i.e. assume you start with a model $\hat{f}_0$ trained on $D_0$}
% We start start with model $M$ trained on $D_0$ 

% \begin{align}
%     M_0 = \argmin_M \sum_i \ell(f_0(x_i), M(x_i))
% \end{align}
% \fk{I probably need to add $\theta$, also we cannot exactly compute the argmin}

% We now demonstrate how users can interact with the model ($M_0$) to apply their concepts (i.e., update the model in a way that model would have good performance in their domain) without interfering with each other's concepts or reducing the performance of the model on $\sP_0$.
% Specifically, in Section~\ref{debugging}, we show how we can assist users in conceptualizing their concepts within the context of our model, including identifying, generalizing, and fixing bugs in the model; and in Section~\ref{interference}, we demonstrate how to effectively manage interference between concepts. Our ultimate goal is to infer $M_{0:k}$, a model with low error on all concepts.

\subsection{Conceptualizing concepts and debugging}
\label{sec:debugging}
% In this section, for a single user $u_i$ we first explain how to find a bug in the model with few queries from user (i..e, finding $x \in C_i$ that $M_0(x) \neq f(x)$)
% \todo[inline]{'Find a bug' came out of nowhere. Why do I want to find a bug?}
% We then explain how to update the model to have good performance in the user domain. 

% In particular, in Section~\ref{sec:random-walk} we create a Markov chain using $\sG$ which allows for exploration in the user domain, We then in section~\ref{sec:hill-climb} show that given a score function we can search the user domain more efficiently for a data point that maximize that score, finally in Section~\ref{sec:local-inference}, we show how to infer such score function and provide the final algorithm for debugging part of \method{}.
% \todo[inline]{Signposting is only good if the reader need to keep the structure in mind when reading the next thing, and the structure is not obvious.}

\subsubsection{Markov Chain}
\label{sec:random-walk}
%how does MC work
\todo[inline]{Make sure to mention here why we need user + LLM}
The main challenge is that we cannot sample from $\sP_i$.
In order to address this challenge we use the generator $\sG$ to create a Markov chain to simulate a random walk within the user's distribution ($\sP_i$). 
Specifically, we begin with a user-provided seed data point $x$ and use it as a prompt for $\sG$ to generate a new data point $x'$. If $\sP_i(x') >0$, we accept $x'$, otherwise we remain at $x$ and repeat the process. 

%connectivity is important
In Appendix~\ref{sec:app} we study conditions under which the stationary distribution of this Markov chain is $P_i$. However, note that we do not need this condition to find bugs during random walk we only need connectivity according to the transition function $\sP'$ which means for any $x_1, x_n \in C_i$ there exists $x_2, \dots, x_{n-1} \in C_i$ such that $\Pi_{i=1}^{n-1} \sP'(x_{i+1} \mid x_{i}) > 0$, Given this condition we will find bugs after enough explorations. 

%exploration -> more rejection but cover more of user domain, explotation -> less reject, less query
\paragraph{Uncovered error.} 
% In order to make the $\sG$ transitions more aligned with the $\sP_i$ we can do a better prompt engineering by adding some information about the concept to the prompt, or adding multiple data points instead of only one. 
Depending on the prompt we can make the probability of generating in-domain for a concept lower but having high recall (e.g., only using 1-2 data points as prompt). Or, we can make the prompt more specific (e.g., adding some info and 10 data points) and increase the probability of generation in-domain but decrease the recall.  
% In this work following \cite{ribeiro2022adaptive} we realized that instead of one data point for the prompt from a domain we can use $3-7$ data points  and then do the random walk as explained above, in this case we decrease the probability of generating out of concept data point with the risk of not being able to reach some data points. Note that we can still define a new graph with any $3-7$ data points as a node and define our Markov Chain on the new graph.
% %not covered at all! (moves to discusion?)
% There also might be some data points are not represented in the $\sG$ corpus so we cannot reach them using prompt-engineering by $\sG$ to them while they are in the user domain. 
% Furthermore, it is possible that user domain is not connected according to the transition function of $\sG$. Stronger $\sG$ (e.g., Advancement in language models) and having a strong seed data points (i.e., diversity among users) can help with this errors.

\subsubsection{Learning a Local Model}
\todo[inline]{Why local model}
\label{sec:local-inference}
%introduction
Previous section showed that how to utilize the generator ($\sG$) to find to traverse the user's domain. However, this involves asking user many questions. 
We now try to create a function as the proxy for the user so we can decrase the amount of queries from user.
In order, to so we use the fact that complicated functions can be approximated in a local neighborhood with a simpler function (e.g., first few terms of a Taylor series). Therefore, we assume $f$ has a simple form in $C_i$. 
We call this local function $f_i$ (the local function $f_i$ has perfect alignment with $f$ in $C_i$ but can be very different from $f$ everywhere else). 
A good characteristic of simple functions is that we can learn them in isolation with only a few samples.

%example
As an example consider $\sP_0$ to be a mixture of two elliptical Gaussian with one component per class as shown in top of the  Figure~\ref{fig:interference_linear}(a), while the user $i$ concept is a mixture of two spherical Gaussian with one component per class as shown at the bottom of Figure~\ref{fig:interference_linear}(a). 
As $M_0$ is only trained on the top two elliptical Gaussian it is tilted (the dashed line) compare to the true classifier (solid line) which leads to some bugs in the user concept (spherical Gaussian). 
We want to find regions in $C_i$ that are prone to be bug. 
In order to do so, we first learn a linear classifier for spherical Gaussian in isolation. Since learning concepts in isolation requires less data, we can learn a classifier with high accuracy only with a few data points as shown Figure~\ref{fig:interference_linear}(b). 
We then define the score function as disagreement between these two models.
Figure~\ref{fig:interference_linear}(c) shows the regions with high disagreements (therefore, more prone to bug).
\todo[inline]{This argument seems a little handwaivy?}



%fixing & algorithm
Now that we find an efficient way of finding bugs we update the local and global models whenever we find a disagreement.
Although local models are usually have higher accuracy in the user's domain than the global model as they are only optimizing the user's domain they might miss some part of the user's concept as they are only trained on a very few data points. 
As a result, whenever we find a disagreement we either make the local function a better proxy of the labeling function of the user ($f_i$) or it is truly a bug in the model and we update the model. 

%exploration -> more asking question even when score is low but find more bus, explotation -> less asking low score, less query
\paragraph{False agreements.} 
In \ref{sec:local-inference} we infer a local function that serve as a proxy for the user, however this local function is not always right (as it is possible that local and global agree but the label is wrong). Depending on how much we rely on the local function (e.g, how do we sample data points to show the user) we can do a trade-off between precision-recall for bugs. 


\subsubsection{Hill Climbing}
\todo[inline]{Why global model probably goes here or in the next}
\label{sec:hill-climb}
%explain hill-climb
We need to use $\sG$ a lot to find a data point in disagreement region of local and global function. 
Can we make this process more efficient?
We define a score function as the disagreement between local and global function and our goal is to find $x$ to maximize this function. 
We now adapt the random walk such that we find the maximum of this function therefore finding bugs sooner and asking user less queries about membership
We are only enable to do local search while we are interested in global maximum, Hill climbing \cite{} and simulated annealing \cite{} are the common ways to deal with this optimization problem, as we need to do some exploration-exploitation trade-off. 

%special cases
For special cases, we can prove that we can find the global maximum. For example, when the score function is linear and domain of the user is convex, and the generator $\sG$ samples according to power low, \cite{Adam} has proved that we only need $\sO(n^{4.5})$ to find the global maximum (where $n$ is the dimension of the space). 

%exact case of our algorithm
\ref{alg:hill-climb} shows how we do exploration and exploration to find the maximum of a score function in a specific domain $\sP_i$. 


%exploration -> more asking question even when score is low but find more bus, explotation -> less asking low score, less query
\paragraph{Local maximum.}  
It is possible that we get stuck in the local maximums. in this case we can explore more while asking user more question.
%foldering so we do not stuck in local maximum
In addition we allow user to group data points together so users can interactively group data points together so stop stucking in one place and make the $\sG$ to explore other regions.
As a final note, we also allow user to group data points together, we then in the generation step in addition to sample according to the score function we also keep into account the distance from the current folders. This allow user to not get stuck in the local maximum and also find a diverse set of bugs. 
\todo[inline]{I doubt any reader will grasps what this means at this point, should probably abstract away the notion of subtopics and mention it somewhere else}

\subsubsection{\method-Debugging}

Putting everything together our final algorithm for teaching a model about a concept is as follows:
\begin{enumerate}
    \item {\bf Seed session:}  The user provides a few examples from her concept and their labels called $D_i$.
    \item {\bf Local fit:}  Set $M_{i0} = M_0$, We locally fit $M_i$ to $D_i$.
    \item {\bf Generation:} We choose a subset of $D_i$ and using $\sG$ to generate new data points with hill climbing toward $score(x) = M_{i:0}(x) - M_i(x)$
    \item {\bf Selection:} We select a set of data points that $M_i, M_{i0}$ disagree with each other. We ask user $u_i$ to resolve the conflict. We then add the new data points to $D_i$. 
    \item {\bf Update:} If the user still can find errors go directly to step 2, if the user could not find any error this round then update $M_{i0}$ by training it on $D_0 \cup D_i$, update $M_i$ by training it on $D_i$ and then go to step 2, if $D_i$ has not changed from the previous round then quit.
\end{enumerate}

%types of bugs
For each disagreement between global and local function, there are two possibilities: 
\begin{enumerate}
    \item $M_i$ is relying on some shortcuts that is not correct for this data point and $M_{i0}$ is the correct label, in this case user update the model it helps the user to conceptualize its model better and make the local model better represent $f_i$.
    \item $M_{i}$ is predicting the correct label and $M_{i0}$ predicts wrongly on this data point, this is true bug in the model and as we update the model we lead $M_{i0}$ to have a better representaion of $f_i$ in the concept of user $i$ ($C_i$). 
\end{enumerate} 
The user handles this disagreement on step 3 and clarify which possibility is correct. Figure~\ref{fig:debugging} shows the pipeline of \method{} for debugging of a model for a single user. 

%active learning and false-agreements & exploration-exploitation
If local and global model align with each other, then due to randomness in seed they might disagree with each other near boundary and our method start to work like active-learning. 
There is a possibility that both local and global model agree on some data points confidently with the wrong function which we call \emph{false agreement}, we can show the user some data points to label even if local and model do not disagree to deal with this type of error. In the next section we discuss the knobs that we have for exploration vs. exploration.


%why not pure active learning?
%we beilive there is a big overlap between user function and the global function we study this more in LR-analysis. 




% \subsubsection{Exploration-Exploitation trade-offs}
% \todo[inline]{Fold this back in the previous subsection}

% The debugging part of \method{} has three components in each component we can do trade-off between exploration (which leads to more discovery of bugs but more query from the user) and exploitation (where lead to less discovery of bugs but also less query from the user). 

 




\input{debugging_figure}
\input{psudo_conflict}

\subsection{Handling interference}
\label{sec:interference}
%introduction
In previous section, we show that how \method{} enables users to conceptualize their concepts and improve the performance of the base model in their domains. 
However, any changes made to one part of the model can have an impact on the overall model.
%intuition
For example, \reffig{interference_intuition} compare the first and last figure in Figure~\ref{fig:debugging} and shows that when we update the model to satisfy the constraint of user $i$ (the black circle) it causes change in the domain of user $j$ (black square) or the original distribution outside any concept (top right corner).  
In this section, We show how \method{} deals with multiple users and manage their interference effectively results in better performance for all users. \todo[inline]{Should probably talk about multiple concepts rather than multiple users?} \fk{In our setup we defiend $k$ users so let's go with that?}
 
%interference with previous models 
Let $M_{0:i-1}$ denote a model trained on $D_{0:i-1}$ and works well in all $0$ to $i-1$ domain. Now $u_i$ wants to update the model with $D_i$ that gather with interaction with $M_{0:i-1}$ as explained in Section~\ref{sec:debugging}. 
The new change might interfere with previous user's concepts. However, since every user has a local model that works well in their domain after each change we check with the previous models and see if the new change has created a new interference in their domain.


%interference with original model
For the conflict with original model, we assume $D_0$ has enough data points so $M_0$ does not rely on any shortcuts in its own domain ($\sP_0$). Therefore, for disagreement on $\sG(D_0)$ we assume that local model is always correct and $M_0$ predicts the correct label. 
In experiment section, when we have access to a lot of training data, we only sample training data that the new global model predict differently and add them to the $D_0$ for fine-tunning. 
% Therefore, we do a self-training on $D_0$ before the procedure to not loose accuracy.
% {\bf Self-Training:} For each $x \in \sG(D_0)$ create a data point $(x, M_0(x))$ and add it to $D_0$.

%interference as opportunity
Interference can be beneficial by exposing false agreement bugs (Section!\ref{sec:type-of-errors}) in previous models. For example, the local model of the user $i$ might only focuses on color to distinguish between oranges and bananas may have a shortcut. A global model that doesn't have any other objects with the color yellow or orange may also rely on color as a shortcut. When a new concept, such as a lemon, is introduced, it can cause interference between the new global and the local model for user $i$, revealing the shortcut in their local function.


%some general notes
In general now we can pick any two users and check if the dataset from one user conflict the model for another user. Formally, for $u_i$ and $u_j$ we can check conflicts between $M_i$ and $M_{ij}$ on $\sG(D_i)$ using the hill-climb algorithm with the score as the disagreement between $M_i$ and $M_{ij}$. Using this technique we can 
Also we can include the distance between embedding of data points in $u_i$ to the embedding data point in $u_j$ to incentives the hill-climb to generate sentences in $C_i$ near $C_j$. 



==> psudo_conflict.tex <==
% \begin{algorithm}
%     \caption{Hill-climb (Score, D)}
%     \label{algo:interference}
%     \begin{algorithmic}
%         \FOR{$L$ iteration}
%             \STATE {\bf sampling:} Sample $7$ data point according to their $score(x)$
%             \STATE {\bf generation} prompt $\sG$ with the candidate and add the $k$ new generation and add them to the candiates.
%             \STATE {\bf selection} select candidates thate are promising and ask uer to see if $p_i(x) > 0$
%         \ENDFOR
%     \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}
%     \caption{Resolving Disagreements between $M_S$ and $M_T$ on $D_i$}
%     \label{algo:interference}
%     \begin{algorithmic}
%         \FOR{$L$ iteration}
%             \STATE {\bf Generation:} Generate a list of candidate using $\sG$ and $D_i$ by hill climbing toward the maximum disagreements between $M_S$ and $M_T$
%             \STATE {\bf Selection:} Select some of data points that $M_S$ and $M_T$ disagree and ask user for their true label and add them to $D_i$
%             \STATE {\bf Update:} update $M_S$ and $M_T$ with $D_i$
%         \ENDFOR
%     \end{algorithmic}
% \end{algorithm}

\fk{non-of these algorithm box makes sense! I'm just trying to decide if we need one or not}
\begin{algorithm}
    \caption{Hill-climb (Score, D)}
    \label{algo:interference}
    \small
        \For{$L$ iteration}
        {
            {\bf sampling:} Sample $7$ data point according to their $score(x)$ \;
             {\bf generation} prompt $\sG$ with the candidate and add the $k$ new generation and add them to the candiates. \;
             {\bf selection} select candidates thate are promising and ask uer to see if $p_i(x) > 0$ \;
        }
\end{algorithm}


\begin{algorithm}
    \caption{Resolving Disagreements between $M_S$ and $M_T$ on $D_i$}
    \label{algo:interference}
    \small
        \For{$L$ iteration}{
             {\bf Generation:} Generate a list of candidate using $\sG$ and $D_i$ by hill climbing toward the maximum disagreements between $M_S$ and $M_T$ \;
             {\bf Selection:} Select some of data points that $M_S$ and $M_T$ disagree and ask user for their true label and add them to $D_i$ \;
             {\bf Update:} update $M_S$ and $M_T$ with $D_i$ \;
        }
\end{algorithm}


\begin{algorithm}
\DontPrintSemicolon
    \caption{Handling Interference}
    \label{algo:interference}
    \small
        \For{$i=1$ to $n$}
        {
            \tcc{first result disagreement between $i$ and $0$}
            { $D_i$ is the seed data from user $i$}\;
            { Resolve disagreements between $\hat{f}_{0:i}$ and $\hat{f}_{i}$ in domain $i$}\;
            \While{True}
                {
                \For{$j=0$ to $i$}
                    {
                     {Add disagreements between $\hat{f}_{j}$ and $\hat{f}_{0:i}$ in domain $j$ to $D_j$}
                    }
                Fine-tune $M_{0}$ on $D_{0:i}$ \;
                For all $j$ infer $M_j$ using $D_j$ \;
                \If{No new data has been added to any $D$}
                    {
                     break
                    }
                }
        }
\end{algorithm}
